BERT, can HE predict contrastive focus? Predicting and controlling prominence in neural TTS using a language model

Several recent studies have tested the use of transformer language model representations to infer prosodic features for text-to-speech synthesis (TTS). While these studies have explored prosody in general, in this work, we look specifically at the prediction of contrastive focus on personal pronouns. This is a particularly challenging task as it often requires semantic, discursive and/or pragmatic knowledge to predict correctly. We collect a corpus of utterances containing contrastive focus and we evaluate the accuracy of a BERT model, finetuned to predict quantized acoustic prominence features, on these samples. We also investigate how past utterances can provide relevant information for this prediction. Furthermore, we evaluate the controllability of pronoun prominence in a TTS model conditioned on acoustic prominence features.

==> table-old.tex <==

\begin{table*}[t]
 \caption{Results for the prominence prediction task for the $<$p2$>$ (high prominence) category. F1, Recall (R) and Precision (P) are reported for the full test set (all POS categories combined). Recall is reported for the two manually verified subsets of contrastively focused personal pronoun. }
 \label{tab:predictionResults}
\begin{tabular}{lllllllllllll}
\hline
\textbf{Model} & \textbf{Testset}  & \multicolumn{3}{l}{\textbf{Current Sentence}} & \multicolumn{3}{l}{\textbf{Prev Sentence}} & \multicolumn{3}{l}{\textbf{2 Prev Sentences}} & \textbf{\# p2} & \textbf{\# words} \\ \hline
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \textbf{\footnotesize F1 p2} & \textbf{\footnotesize R p2} & \textbf{\footnotesize P p2} & \textbf{\footnotesize F1 p2} & \textbf{\footnotesize R p2} & \textbf{\footnotesize P p2} & \textbf{\footnotesize F1 p2} & \textbf{\footnotesize R p2} & \textbf{\footnotesize P p2} &  &  \\ \hline
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\footnotesize Full testset} & \footnotesize 0.458 & 0.394 & 0.546 & \multicolumn{6}{l}{\cellcolor[HTML]{EFEFEF}} \footnotesize & 79,793 & 365,330 \\
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\footnotesize Pronoun maj.} &  & 0.079 &  & \multicolumn{6}{l}{\cellcolor[HTML]{EFEFEF}} & 393 & 393 \\
\multicolumn{1}{l|}{\multirow{-3}{*}{\textbf{Word Majority}}} & \multicolumn{1}{l|}{\footnotesize Pronoun min.} &  & 0.000 &  & \multicolumn{6}{l}{\multirow{-3}{*}{\cellcolor[HTML]{EFEFEF}}} & 100 & 100 \\ \hline
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\footnotesize Full testset} \footnotesize & 0.572 & 0.539 & 0.609 & 0.565 & 0.546 & 0.586 & 0.561 & 0.558 & 0.565 & 79,793 & 365,330 \\
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\footnotesize Pronoun maj.} &  & 0.178 &  &  & 0.160 &  &  & 0.135 &  & 393 & 393 \\
\multicolumn{1}{l|}{\multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Randomly \\Initialized BERT\end{tabular}}}} & \multicolumn{1}{l|}{\footnotesize Pronoun min.} &  & 0.06 &  &  & 0.06 &  &  & 0.06 &  & 100 & 100 \\ \hline
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\footnotesize Full testset} \footnotesize & \footnotesize 0.588 & \footnotesize 0.552 & \footnotesize 0.629 & \footnotesize 0.580 & \footnotesize 0.536 & \footnotesize 0.632 & \footnotesize 0.579 & \footnotesize 0.535 & \footnotesize 0.629 & \footnotesize 79,793 & \footnotesize 365,330 \\
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\footnotesize Pronoun maj.} &  & 0.239 &  &  & 0.239 &  &  & 0.216 &  & 393 & 393 \\
\multicolumn{1}{l|}{\multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}BERT fine-tuned \\ on CWT features\end{tabular}}}} & \multicolumn{1}{l|}{\footnotesize Pronoun min.} &  & 0.06 &  &  & 0.07 &  &  & 0.07 &  & 100 & 100 \\ \hline
\end{tabular}
\end{table*}


==> table-pronouns.tex <==
\begin{table*}[]
 \caption{Results on pronouns only for the prominence prediction task. Recall is reported for the two manually verified subsets of contrastively focused personal pronouns and the non-contrastive pronoun subset (Neg: 493 samples). Maj: group of 393 samples where majority of speakers used contrastive focus. Min: group of 100 samples where only 1 out of 3 speakers used contrastive focus.}
 \label{tab:pronouns}
\begin{tabular}{c|c|c|c|c}
\hline
\footnotesize Model                     & \footnotesize Annotation & \footnotesize R (Current Sentence) & \footnotesize R (+Previous Sentence) & \footnotesize R (+2 Prev Sentences) \\ \hline
\footnotesize Word Majority             & \footnotesize Maj        & \footnotesize 0.079               &                        &                      \\
                          & \footnotesize Min        & \footnotesize 0.000               &                        &                      \\ \hline
\footnotesize \footnotesize Randomly Initialized BERT & \footnotesize Maj        & \footnotesize 0.178               & \footnotesize 0.160 & \footnotesize 0.135                \\
                          & \footnotesize Min        & \footnotesize 0.060               & \footnotesize 0.060                  & \footnotesize 0.060                \\ \hline
\footnotesize Fine Tuned BERT           & \footnotesize Maj        & \footnotesize 0.239               & \footnotesize 0.239                  & \footnotesize 0.216                \\
                          & \footnotesize Min        & \footnotesize 0.060               & \footnotesize 0.070                  & \footnotesize 0.070                \\ \hline
\end{tabular}
\end{table*}



